UnNatural Language Inference

Recent investigations into the inner-workings of state-of-the-art large-scale pre-trained Transformer-based Natural Language Understanding (NLU) models indicate that they appear to know humanlike syntax, at least to some extent. We provide novel evidence that complicates this claim: we find that state-of-the-art Natural Language Inference (NLI) models assign the same labels to permuted examples as they do to the original, i.e. they are largely invariant to random word-order permutations. This behavior notably differs from that of humans; we struggle with ungrammatical sentences. To measure the severity of this issue, we propose a suite of metrics and investigate which properties of particular permutations lead models to be word-order invariant. In the MNLI dataset, for example, we find almost all (98.7%) examples contain at least one permutation which elicits the gold label. Models are sometimes even able to assign gold labels to permutations that they originally failed to predict correctly. We provide a comprehensive empirical evaluation of this phenomenon, and further show that this issue exists for both Transformers and pre-Transformer RNN / ConvNet based encoders, as well as across multiple languages (English and Mandarin Chinese). Our code and data are available at https://github.com/facebookresearch/unlu.

==> tables/nli_rand_nt.tex <==
\begin{table}[ht]
    \centering
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{@{}llrrrrr@{}}
            \toprule
     Model &    Eval Dataset &  $\mathcal{A}$ &  $\Omega_{\text{max}}$ &  $\mathcal{P}^c$ &  $\mathcal{P}^f$ &  $\Omega_{\text{rand}}$ \\
\midrule
 \multirow{7}{*}{\bf InferSent} 
 &   MNLI\_m\_dev &              0.658 &         0.904 &                  0.842 &             0.359 &                        0.712 \\
 &  MNLI\_mm\_dev &              0.669 &         0.905 &                  0.844 &             0.368 &                        0.723 \\
 &     SNLI\_dev &              0.556 &         0.820 &                  0.821 &             0.323 &                        0.587 \\
 &    SNLI\_test &              0.560 &         0.826 &                  0.824 &             0.321 &                        0.600 \\
 &  A1\_dev &              0.316 &         0.669 &                  0.425 &             0.395 &                        0.313 \\
 &  A2\_dev &              0.310 &         0.662 &                  0.689 &             0.249 &                        0.330 \\
 &  A3\_dev &              0.300 &         0.677 &                  0.675 &             0.236 &                        0.332 \\ \midrule
 & Mean &  \textbf{0.481} & 0.780 & 0.731 & \boldred{0.322} & 0.514 \\ 
 & Harmonic Mean &  0.429 & 0.767 & 0.694 & \boldred{0.311} & 0.455 \\ \midrule
 \multirow{7}{*}{\bf ConvNet}
 &   MNLI\_m\_dev &              0.631 &         0.926 &                  0.773 &             0.340 &                        0.684 \\
 &  MNLI\_mm\_dev &              0.640 &         0.926 &                  0.782 &             0.343 &                        0.694 \\
 &     SNLI\_dev &              0.506 &         0.819 &                  0.813 &             0.339 &                        0.597 \\
 &    SNLI\_test &              0.501 &         0.821 &                  0.809 &             0.341 &                        0.596 \\
 &  A1\_dev &              0.271 &         0.708 &                  0.648 &             0.218 &                        0.316 \\
 &  A2\_dev &              0.307 &         0.725 &                  0.703 &             0.224 &                        0.356 \\
 &  A3\_dev &              0.306 &         0.798 &                  0.688 &             0.234 &                        0.388 \\ \midrule
 & Mean &  0.452 & \boldred{0.817} & \boldred{0.745} & 0.291 & 0.519 \\ 
& Harmonic Mean &  0.404 & \boldred{0.810} & \boldred{0.740} & 0.279 & \boldred{0.473} \\ \midrule
 \multirow{7}{*}{\bf BiLSTM} 
 &   MNLI\_m\_dev &              0.662 &         0.925 &                  0.800 &             0.351 &                        0.711 \\
 &  MNLI\_mm\_dev &              0.681 &         0.924 &                  0.809 &             0.344 &                        0.724 \\
 &     SNLI\_dev &              0.547 &         0.860 &                  0.762 &             0.351 &                        0.598 \\
 &    SNLI\_test &              0.552 &         0.862 &                  0.771 &             0.363 &                        0.607 \\
 &  A1\_dev &              0.262 &         0.671 &                  0.648 &             0.271 &                        0.340 \\
 &  A2\_dev &              0.297 &         0.728 &                  0.672 &             0.209 &                        0.328 \\
 &  A3\_dev &              0.304 &         0.731 &                  0.656 &             0.219 &                        0.331 \\ \midrule
 & Mean &  0.472 & 0.814 & 0.731 & 0.301 & \boldred{0.520} \\
& Harmonic Mean &  0.410 & 0.803 & 0.725 & 0.287 & 0.463 \\
 
\bottomrule
        \end{tabular}}
    \caption{Statistics for Non-Transformer Models. All models are trained on MNLI corpus \cite{williams-etal-2018-broad}. $\Omega_{\text{max}}$ or Max accuracy is computed if \textit{any} of the $n=100$ permutations per data point yield correct results. $\mathcal{P}^c$  stands for the mean number of permutations which were correct when the original prediction is correct. $\mathcal{P}^f$  stats for the mean number of permutations which are correct when the original prediction is incorrect (flip). $\Omega_{\text{rand}}$ is computed as the percentage of data points the ground truth label is chosen over a random uniform baseline (1/3). Bold marks the highest value per metric (\boldred{red} shows  the model is insensitive to permutation).}
    \label{table:main_non_t}
\end{table}

